Continuous Relaxation of Symbolic Planner for One-Shot Imitation Learning

We address one-shot imitation learning, where the goal is to execute a previously unseen task based on a single demonstration. While there has been exciting progress in this direction, most of the approaches still require a few hundred tasks for meta-training, which limits the scalability of the approaches. Our main contribution is to formulate one-shot imitation learning as a symbolic planning problem along with the symbol grounding problem. This formulation disentangles the policy execution from the inter-task generalization and leads to better data efficiency. The key technical challenge is that the symbol grounding is prone to error with limited training data and leads to subsequent symbolic planning failures. We address this challenge by proposing a continuous relaxation of the discrete symbolic planner that directly plans on the probabilistic outputs of the symbol grounding model. Our continuous relaxation of the planner can still leverage the information contained in the probabilistic symbol grounding and significantly improve over the baseline planner for the one-shot imitation learning tasks without using large training data.

==> 0_preamble.tex <==
% Author: Animesh Garg
% Date : July 2015
% This is a list of common packages needed in a wide range of latex docs for everyday writing.
% ---------------------------------
%floats and figures
% ---------------------------------
\usepackage{graphics}
\usepackage[pdftex]{graphicx}
\usepackage{wrapfig}
\DeclareGraphicsExtensions{.pdf,.png,.jpg}
%\pdfimageresolution200
\usepackage{epsfig}
\usepackage[font={small}]{caption}
\usepackage{subcaption}
%DONT USE BOTH SUBCAPTION AND SUBFIGURE
%\usepackage[center]{subfigure} 
% \usepackage{overpic}
\usepackage[rightcaption]{sidecap}
\usepackage{pbox}

\usepackage{bigstrut}
\setlength\bigstrutjot{3pt}

% ---------------------------------
%Math Stuff
% ---------------------------------
\usepackage{mathtools}
\usepackage{amsmath, amssymb, amscd}
\usepackage{ wasysym } %special symbols
\usepackage{amsfonts}
\usepackage{mathptmx} % selects Times Roman as basic font
\usepackage{gensymb} 
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{mdwmath}
% \usepackage{mdwtab}
% \usepackage{eqparbox} %equations
% \usepackage{mathtools}
\numberwithin{equation}{section} 

% ---------------------------------
%Symbols
% ---------------------------------
\DeclareMathAlphabet{\mathcal}{OMS}{lmsy}{m}{n}
\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
\usepackage{textcomp} %for getting text tilde
%\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
%\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
%\usepackage{dsfont}

% ---------------------------------
%  Algorithms
% ---------------------------------
% http://tex.stackexchange.com/questions/229355/algorithm-algorithmic-algorithmicx-algorithm2e-algpseudocode-confused

\usepackage{algorithm} %float wrapper for algorithms. %dont use with algorithm2e
%should only use one of algorithmic or algorithmicx or algorithm2e
% \usepackage{algorithmic} %least preferred
% \usepackage[ruled,vlined,linesnumbered]{algorithm2e} 
\usepackage{algorithmicx, algpseudocode} %algpseudocode:layout for algorithmicx

% \algtext*{EndFunction}% Remove "end while" text
% \algtext*{EndWhile}% Remove "end while" text
% \algtext*{EndIf}% Remove "end if" text


% ---------------------------------
%Table Stuff
% ---------------------------------
\usepackage{array} %for table entries to be in center of cell
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{booktabs}
\usepackage{tabulary}

% ---------------------------------
%DOCUMENT WIDE
% ---------------------------------
\usepackage[T1]{fontenc} 
\usepackage[utf8]{inputenc}
\usepackage[english]{babel} %for hyphenation rules
\usepackage{units}
% \usepackage{siunitx}
\usepackage{bm}
\usepackage{times} % assumes new font selection scheme installed
\usepackage{xspace}
\usepackage{flushend}%balance columns on last page
\usepackage{balance} 
\usepackage{csquotes}
\usepackage{makeidx}
\usepackage{blindtext}

\let\labelindent\relax
\usepackage{enumitem}

\usepackage{tikz}
\usetikzlibrary{backgrounds}

\usepackage{ragged2e}
% \usepackage{fixltx2e} %fix latex issue across versions not needed in new latex versions
\usepackage{soul} %text highlighting
\usepackage{subfiles} %individual file compilation--makes it quick 

\usepackage[protrusion=true,expansion=true]{microtype}
\setlength{\emergencystretch}{3em}

\usepackage[yyyymmdd]{datetime}
\renewcommand{\dateseparator}{-}
\date{\protect\formatdate{1}{1}{2001}}

% ---------------------------------
%Bibliography and cross-ref
% ---------------------------------
% The following lines are for IEEE style conflicts with natbibs
% \makeatletter
% \let\NAT@parse\undefined
% \makeatother
% \usepackage[numbers]{natbib}
% \usepackage{cite} %DONT USE NATBIB AND CITE TOGETHER

%hyperlinking
\usepackage{url}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother
\usepackage{color}
% \usepackage[usenames,dvipsnames,table]{xcolor}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}

% \usepackage[pdfborder={0 0 0.5}]{hyperref}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=black,
    citecolor=black,
    filecolor=cyan,
    urlcolor=black
}

%=======U S E R  D E F I N E D  M A C R O S=======
% ---------------------------------
% User Comments
% ---------------------------------
\usepackage{marginnote}
% \newcommand{\bibhref}[2]{#2}
\usepackage{soul} %text highlighting
\newcommand{\todohl}[1]{{[\hl{#1?}]}}

%\usepackage[disable]{todonotes}
% \usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
\renewcommand{\todo}[1]{\textcolor{red}{[#1?]}}
%takes in optional argument
\newcommand{\tocite}[1]{%
\textcolor{red}{[cite:\ifthenelse{\equal{#1}{}}{}{#1}?]}
}

% \newcommand\todo[1]{{\color{red} TODO: #1 }}

\newcommand{\ignore}[1]{}
\newcommand{\etal}{et al.~}

\newcommand{\ie}{\emph{i.e., }}
\newcommand{\eg}{\emph{e.g., }}

%version in control in draft mode
\newcommand{\versionString}{\textcolor{red}{draft-mode-[\today\ \currenttime]}}

% ---------------------------------
% Label utils
% ---------------------------------

% Usage:
% \figlabel{myfigure} creates \label{fig:myfigure}
% \figref{myfigure} references it
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\figref}[1]{Figure\,\ref{fig:#1}}

% Usage:
% \seclabel{mysection} creates \label{sec:mysection}
% \secref{mysection} references it
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Section\,\ref{sec:#1}}

\newcommand{\chlabel}[1]{\label{ch:#1}}
\newcommand{\chref}[1]{Chapter\,\ref{ch:#1}}

% Usage:
% \tablabel{mytable} creates \label{tab:mytable}
% \tabref{mytable} references it
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

\newcommand{\eqnref}[1]{{Eq.\ (\ref{eq:#1})}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% space tweaks 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setlength{\abovecaptionskip}{1mm}        
\setlength{\belowcaptionskip}{0mm}        
\setlength{\textfloatsep}{0mm}
\setlength{\dbltextfloatsep}{3mm}
\renewcommand{\baselinestretch}{1.0}

\makeatletter
\newenvironment{mcases}[1][l]
 {\let\@ifnextchar\new@ifnextchar
  \left\lbrace
  \def\arraystretch{1.2}%
  \array{@{}l@{\quad}#1@{}}}
 {\endarray\right.}
\makeatother
